Safe Non-Stochastic Control of Linear Dynamical Systems

We study the problem of \textit{safe control of linear dynamical systems corrupted with non-stochastic noise}, and provide an algorithm that guarantees (i) zero constraint violation of convex time-varying constraints, and (ii) bounded dynamic regret, \ie bounded suboptimality against an optimal clairvoyant controller that knows the future noise a priori. The constraints bound the values of the state and of the control input such as to ensure collision avoidance and bounded control effort. We are motivated by the future of autonomy where robots will safely perform complex tasks despite real-world unpredictable disturbances such as wind and wake disturbances. To develop the algorithm, we capture our problem as a sequential game between a linear feedback controller and an adversary, assuming a known upper bound on the noise's magnitude. Particularly, at each step $t=1,\ldots, T$, first the controller chooses a linear feedback control gain $K_t \in \calK_t$, where $\calK_t$ is constructed such that it guarantees that the safety constraints will be satisfied; then, the adversary reveals the current noise $w_t$ and the controller suffers a loss $f_t(K_t)$ -- \eg $f_t$ represents the system's tracking error at $t$ upon the realization of the noise. The controller aims to minimize its cumulative loss, despite knowing $w_t$ only after $K_t$ has been chosen. We validate our algorithm in simulated scenarios of safe control of linear dynamical systems in the presence of bounded noise

==> Alg/Alg-SafeAder-Control.tex <==
%\setlength{\textfloatsep}{-0.5mm}
% \setlength{\aboveskip}{0mm}
\begin{algorithm}[t]
	\caption{\hspace{-.05mm} Safe Adaptive Learning for Dynamic Environment (\SafeAder) for \SafeNSC (\Cref{prob:SafeNSC}).}
	\begin{algorithmic}[1]
		\REQUIRE Time horizon $T$; number of base-learners $N$ per \cref{eq:SafeAder_N_control}; step-size pool $\calH$ per \cref{eq:SafeAder_step_size_pool_control}; initial weight of base-learners $\boldsymbol{p}_{1}$ per \cref{eq:SafeAder_initial_weight_control}; learning rate $\epsilon$ for meta-algorithm per \cref{eq:SafeAder_meta_step_size_control}.
		\ENSURE Control $u_t$ at each time step $t=1,\ldots,T$.
		\medskip
		\STATE Initialize ${K}_{1,i} \in \calK_1$, $\forall i \in \{1, \dots, N\}$; 
		\FOR {each time step $t = 1, \dots, T$}
		\STATE Receive ${K}_{t,i}$ from base-learner $\calB_i$ for all $i$;
		\STATE Calculate ${K}_t = \sum_{i=1}^{N}p_{t,i}{K}_{t,i}$;
		\STATE Output $u_t = -K_t x_t$;
        \STATE Observe the state $x_{t+1}$ and calculate the noise $w_t = x_{t+1} - A_t x_t - B_t u_t$;
		\STATE Observe the loss function $c_t: \mathbb{R}^{d_x} \times \mathbb{R}^{d_u} \mapsto \mathbb{R}$ and suffer the loss $c_t(x_{t+1}, u_t)$;
            \STATE Express the loss function in $K_t$ as $f_t({K}_t): \mathbb{R}^{d_u\times d_x} \mapsto \mathbb{R}$;
		\STATE Obtain gradient $\nabla_K f_t({K}_t)$;
		\STATE Construct the surrogate loss
			% \vspace{-2mm}
			 $${\ell}_t({K})=\left\langle\nabla_K {f}_{t}\left({K}_{t}\right), {K}-{K}_{t}\right\rangle; $$
			 % \vspace{-6mm} 			
		\STATE Update the weight of base-learners $\boldsymbol{p}_{t+1} \in \Delta_{N}$ by
			 % \vspace{-3mm}
			$$p_{t+1,i} = \frac{p_{t,i} e^{-\epsilon \ell_{t}({K}_{t,i})}}{\sum_{j=1}^{N}p_{t,j} e^{-\epsilon \ell_{t}({K}_{t,j})}}; $$
			 % \vspace{-5mm}        
       \FOR {each base-learner $\calB_i$, $i = 1, \dots, N$}
        \STATE Update $K_{t+1,i}^\prime=K_{t,i}- \eta_i \nabla_K f_t(K_t)$;
		\STATE Project $K_{t+1,i} = \Pi_{\calK_{t+1}}(K_{t+1,i}^\prime)$;
		\ENDFOR		
		\ENDFOR
    	\end{algorithmic}\label{alg:SafeAder_Control}
\end{algorithm}

==> Alg/Alg-SafeAder.tex <==
%\setlength{\textfloatsep}{-0.5mm}
% \setlength{\aboveskip}{0mm}
\begin{algorithm}[t]
	\caption{\hspace{-.05mm}Safe Adaptive Learning for Dynamic Environment (\SafeAder).}
	\begin{algorithmic}[1]
		\REQUIRE Time horizon $T$; number of base-learners $N$ per \cref{eq:SafeAder_N}; step-size pool $\calH$ per \cref{eq:SafeAder_step_size_pool}; initial weight of base-learners $\boldsymbol{p}_{1}$ per \cref{eq:SafeAder_initial_weight}; learning rate $\epsilon$ for meta-algorithm per \cref{eq:SafeAder_meta_step_size}.
		\ENSURE Decision $\mathbf{x}_t$ at each time step $t=1,\ldots,T$.
		\medskip
		\STATE Initialize $\mathbf{x}_{1,i} \in \calX_1$, $\forall i \in \{1, \dots, N\}$; 
		\FOR {each time step $t = 1, \dots, T$}
		\STATE Receive $\mathbf{x}_{t,i}$ from base-learner $\calB_i$ for all $i$;
		\STATE Output the decision $\mathbf{x}_t = \sum_{i=1}^{N}p_{t,i}\mathbf{x}_{t,i}$;
		\STATE Suffer a loss $f_t(\mathbf{x}_t)$;
		\STATE Observe the loss function $f_t: \ \calX \mapsto \mathbb{R}$;
		\STATE Construct the surrogate loss
			\vspace{-2mm}
			 $${\ell}_t(\mathbf{x})=\left\langle\nabla {f}_{t}\left(\mathbf{x}_{t}\right), \mathbf{x}-\mathbf{x}_{t}\right\rangle; $$
			 \vspace{-6mm} 			
		\STATE Update the weight of base-learners $\boldsymbol{p}_{t+1} \in \Delta_{N}$ by
			 \vspace{-3mm}
			$$p_{t+1,i} = \frac{p_{t,i} e^{-\epsilon \ell_{t}(\mathbf{x}_{t,i})}}{\sum_{j=1}^{N}p_{t,j} e^{-\epsilon \ell_{t}(\mathbf{x}_{t,j})}}; $$
			 \vspace{-5mm}
        \FOR {each base-learner $\calB_i$, $i = 1, \dots, N$}
        \STATE Update $\myx_{t+1,i}^\prime=\myx_{t,i}- \eta_i \nabla f_t(\myx_t)$;
		\STATE Project $\myx_{t+1,i} = \Pi_{\calX_{t+1}}(\myx_{t+1,i}^\prime)$;
		\ENDFOR		
		\ENDFOR
    	\end{algorithmic}\label{alg:SafeAder}
\end{algorithm}

==> preamble_packages.tex <==

%!TEX root = main.tex

% LC: debug
%==========================================================================
%\usepackage{refcheck}
%\usepackage[notref]{showkeys}
%==========================================================================

% LC: to be used for TRO
%==========================================================================
% \usepackage{mathptmx} % assumes new font selection scheme installed
%\usepackage{times} % assumes new font selection scheme installed
%==========================================================================
\usepackage{comment}
\usepackage{siunitx}
\usepackage{relsize}
\usepackage{ifthen}

\usepackage[caption=false]{subfig}

% \begin{comment}
% % Fancy formatting 
% \usepackage[tracking=false,kerning=true,spacing=true]{microtype}
% \usepackage[caption=false]{subfig}

% \usepackage[style=numeric-comp,sorting=none,firstinits=true, maxnames=3,bibstyle=numeric,abbreviate=false,defernums=true,eprint=false,backend=bibtex]{biblatex}
% \renewcommand{\bibfont}{\footnotesize}
% % \DeclareFieldFormat[article]{pages}{#1}%
% % \DeclareFieldFormat[inproceedings]{pages}{#1}%

% \AtEveryBibitem{%
%   \ifentrytype{article}{%
%     \clearfield{pages}%
%   }{%
%   }%
%   \ifentrytype{inproceedings}{%
%     \clearfield{pages}%
%   }{%
%   }%
% }
% \end{comment}

% \bibliography{commons/bib/strings_long}
% \bibliography{commons/bib/all_only_one_w_pages}
% \bibliography{../../references/references}

% \usepackage[noadjust]{cite}
%\usepackage[vlined,ruled,linesnumbered]{algcompatible}
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{rotating}
\usepackage{color}
\usepackage{enumerate}
\usepackage[T1]{fontenc}
\usepackage{psfrag}
\usepackage{epsfig} % for postscript graphics files
%\usepackage{subfigure}
% \usepackage{hyperref}
\usepackage{booktabs}
\usepackage{graphicx,url}
\usepackage{multirow}
\usepackage{array}
\usepackage{latexsym}
\usepackage{amsfonts}
% \usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{amsthm}
\usepackage{xstring}
%\usepackage[noend]{algorithmic}
\usepackage{multirow}
\usepackage{xcolor}
\usepackage{prettyref}
\usepackage{flexisym}
\usepackage{bigdelim}
\usepackage{breqn} % load this last
\usepackage{listings}
\let\labelindent\relax
\usepackage{enumitem}
\usepackage{xspace}
\usepackage{bm}
\graphicspath{{./figures/}}
\usepackage{tikz}
\usetikzlibrary{matrix,calc}
\usepackage{epstopdf}
\usepackage{tikz-cd}
\DeclareGraphicsExtensions{.eps}
\usepackage{threeparttable}


%\usepackage{amsthm} % math
\usepackage{lineno}


%\usepackage{ifpdf}
% Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% compilation based on whether the output is pdf or dvi.
% usage:
% \ifpdf
%   % pdf code
% \else
%    dvi code
% \fi
% The latest version of ifpdf.sty can be obtained from:
% http://www.ctan.org/tex-archive/macros/latex/contrib/oberdiek/
% Also, note that IEEEtran.cls V1.7 and later provides a builtin
% \ifCLASSINFOpdf conditional that works the same way.
% When switching from latex to pdflatex and vice-versa, the compiler may
% have to be run twice to clear warning/error messages.

% *** GRAPHICS RELATED PACKAGES ***
%
%\ifCLASSINFOpdf
  % \usepackage[pdftex]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../pdf/}{../jpeg/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
%\else
  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
  % will default to the driver specified in the system graphics.cfg if no
  % driver is specified.
  % \usepackage[dvips]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../eps/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.eps}
%\fi


\usepackage{mdwlist}
\let\stditemize\itemize
\let\endstditemize\enditemize
\let\itemize\undefined
\makecompactlist{itemize}{stditemize}

%\let\stdenumerate\enumerate
%\let\endstdenumerate\endenumerate
%\let\enumerate\undefined
%\makecompactlist{enumerate}{stdenumerate}
 

